Improving Students' Academic Performance with AI and Semantic Technologies

Artificial intelligence and semantic technologies are evolving and have been applied in various research areas, including the education domain. Higher Education institutions strive to improve students' academic performance. Early intervention to at-risk students and a reasonable curriculum is vital for students' success. Prior research opted for deploying traditional machine learning models to predict students' performance. In terms of curriculum semantic analysis, after conducting a comprehensive systematic review regarding the use of semantic technologies in the Computer Science curriculum, a major finding of the study is that technologies used to measure similarity have limitations in terms of accuracy and ambiguity in the representation of concepts, courses, etc. To fill these gaps, in this study, three implementations were developed, that is, to predict students' performance using marks from the previous semester, to model a course representation in a semantic way and compute the similarity, and to identify the prerequisite between two similar courses. Regarding performance prediction, we used the combination of Genetic Algorithm and Long-Short Term Memory (LSTM) on a dataset from a Brazilian university containing 248730 records. As for similarity measurement, we deployed BERT to encode the sentences and used cosine similarity to obtain the distance between courses. With respect to prerequisite identification, TextRazor was applied to extract concepts from course description, followed by employing SemRefD to measure the degree of prerequisite between two concepts. The outcomes of this study can be summarized as: (i) a breakthrough result improves Manrique's work by 2.5% in terms of accuracy in dropout prediction; (ii) uncover the similarity between courses based on course description; (iii) identify the prerequisite over three compulsory courses of School of Computing at ANU.

==> design.tex <==
\chapter{Design and Implementation}
\label{cha:design}

Same as the last chapter, give the motivation and the high-level
picture of this chapter to readers, and introduce the sections in this
chapter.

\section{Smart Design}
\label{sec:des-hotpath}

\section{Summary}
Same as the last chapter, summarize what you discussed in this chapter and
be a bridge to next chapter.


==> titlepage.tex <==
\begin{titlepage}
  \enlargethispage{2cm}
  \begin{center}
    \makeatletter
    \Huge\textbf{Improving Students’ Academic Performance with AI and Semantic Technologies} \\[.4cm]
    \Huge\textbf{\thesisqualifier} \\[2.5cm]
    \huge\textbf{Yixin Cheng} \\[9cm]
    \makeatother
    \LARGE
    COMP 8755 Individual Computing Project \\
    % \PackageWarning{report template}{Update your course name!} % delete this line when done
    Supervised by: Dr. Bernardo Pereira Nunes
    
    The Australian National University \\[3cm]
    November 2021

    \vspace*{\fill}
    \makeatletter
        {\fontfamily{lmr}\selectfont\textcopyright}\ Yixin Cheng 2021
        \makeatother
    
  \end{center}
\end{titlepage}

